DoraemonGPT: Toward Understanding Dynamic Scenes with Large Language Models (Exemplified as A Video Agent)

Recent LLM-driven visual agents mainly focus on solving image-based tasks, which limits their ability to understand dynamic scenes, making it far from real-life applications like guiding students in laboratory experiments and identifying their mistakes. Hence, this paper explores DoraemonGPT, a comprehensive and conceptually elegant system driven by LLMs to understand dynamic scenes. Considering the video modality better reflects the ever-changing nature of real-world scenarios, we exemplify DoraemonGPT as a video agent. Given a video with a question/task, DoraemonGPT begins by converting the input video into a symbolic memory that stores task-related attributes. This structured representation allows for spatial-temporal querying and reasoning by well-designed sub-task tools, resulting in concise intermediate results. Recognizing that LLMs have limited internal knowledge when it comes to specialized domains (e.g., analyzing the scientific principles underlying experiments), we incorporate plug-and-play tools to assess external knowledge and address tasks across different domains. Moreover, a novel LLM-driven planner based on Monte Carlo Tree Search is introduced to explore the large planning space for scheduling various tools. The planner iteratively finds feasible solutions by backpropagating the result's reward, and multiple solutions can be summarized into an improved final answer. We extensively evaluate DoraemonGPT's effectiveness on three benchmarks and several in-the-wild scenarios. The code will be released at https://github.com/z-x-yang/DoraemonGPT.

==> DoraemonGPT/tables/ablation_component.tex <==
\setlength\intextsep{5pt}
\begin{table}[t]
\centering
\caption{Analysis of essential components on NExT-QA~\cite{xiao2021next} \texttt{s\_train} (\S\ref{exp:ab_trsm}).}
\label{tbl:ab_memory}
\small
\scalebox{0.92}{
\setlength\tabcolsep{4pt}
\renewcommand\arraystretch{1}
\begin{tabular}{|cc||ccc|c|}
    \hline\thickhline
    \rowcolor{mygray}
 TDM & SDM & Acc$_\text{C}$ & Acc$_\text{T}$ & Acc$_\text{D}$ & Acc$_\text{A}$\\
    \hline\hline
    \checkmark &  & 63.3  & 26.7 & 53.3 & 47.8 \\
      & \checkmark & 53.3 & 23.3 & 46.7 & 41.1 \\
    \rowcolor{mygray1} \checkmark & \checkmark & 96.7  & 46.7 & 53.3 & 65.7 \\
    \hline
\end{tabular}
}

\end{table}

==> DoraemonGPT/tables/blip.tex <==

\begin{table}[t]

\caption{The impact of different BLIP models on NExT-QA~\cite{xiao2021next} \texttt{s\_train} (\S\ref{exp:ab_blip}).}
% \centering
\small

\centering

\setlength\tabcolsep{5pt}
% \renewcommand\arraystretch{1.0}
\begin{tabular}{|c||ccc|c|}
    \hline\thickhline
    \rowcolor{mygray}
Models & Acc$_\text{C}$ & Acc$_\text{T}$ & Acc$_\text{D}$ & Acc$_\text{A}$\\
    \hline\hline
    BLIP-2	& 51.4 & 45.5 & 63.3 & 51.2 \\
    \rowcolor{mygray1} InstructBlip	& 54.7 & 50.4 & 70.3 & 55.7
 \\
        \hline
\end{tabular}

\end{table}

==> DoraemonGPT/tables/rvos.tex <==
\begin{table*}[t]
\small
% \centering
\caption{Comparison of our DoraemonGPT with SOTAs on NExT-QA~\cite{xiao2021next} \texttt{val} (\S\ref{exp:quan}). $\dag$: reimplement using the officially released codes. All LLM-driven systems (LLM agent) use the same LLM, \ie, GPT-3.5-turbo.}
% $*$ denotes our implementation since the authors do not release the codes for video question answering.}
% \label{tbl:sota}
% \resizebox{1.0\textwidth}{!}{
\begin{subtable}{0.65\linewidth}
\centering
% \captionsetup{width=.80\linewidth}
{
    % \setlength\tabcolsep{6pt}
    \scalebox{0.88}{
    \setlength\tabcolsep{4pt}
    \renewcommand\arraystretch{1}\small
    \begin{tabular}{|lr|cc||ccc|cc|}
        \hline\thickhline
        \rowcolor{mygray}
        & Method & \multicolumn{2}{c||}{Publication} & Acc$_\text{C}$ & Acc$_\text{T}$ & Acc$_\text{D}$ & Avg & Acc$_\text{A}$ \\ \hline  \hline %& \texttt{top-5} (\%)
        \multirow{5}{*}{\rotatebox{90}{Sup.}} & HME~\cite{fan2019heterogeneous} & CVPR & 2019 & 46.2 & 48.2 & 58.3 & 50.9 & {48.7}\\
        & VQA-T~\cite{yang2021just} & ICCV & 2021 & 41.7 & 44.1 & 60.0 & 48.6 & {45.3}\\
        & ATP~\cite{buch2022revisiting} & CVPR & 2022 & 53.1 & 50.2 & 66.8 & 56.7 & {54.3}\\
        & VGT~\cite{xiao2022video} & ECCV & 2022 & 52.3 & 55.1 & 64.1 & 57.2 & {55.0}\\
        % & VGT~\cite{xiao2022video} & ECCV & 2022 & 49.7 & 53.3 & 63.7 & 55.6 & {55.6}\\
        & MIST~\cite{gao2023mist} & CVPR & 2023 & 54.6 & 56.6 & 66.9 & 59.3 & {57.2}\\
        % & MIST~\cite{gao2023mist} & CVPR & 2023 & 51.7 & 55.3 & 67.0 & 58.0 & {58.0}\\
%        & DRV~\cite{liu2023video} & TCSVT & 2023 & 54.09 & 57.75 & 65.51 & 57.05\\
%        & DRV~\cite{liu2023video} & TCSVT & 2023 & 54.09 & 57.75 & 65.51 & 57.05\\
        \hline\hline
        \multirow{3}{*}{\rotatebox{90}{agent}} & $^\dag$ViperGPT~\cite{suris2023vipergpt} & ICCV & 2023 & 43.2 & 41.0 & 62.3 & 49.4 & {45.5}\\
        % & $^{*\dag}$ViperGPT~\cite{suris2023vipergpt} & ICCV & 2023 & 33.0  & 40.1 & 48.8 & 40.8 & {40.8}\\
        & $^\dag$VideoChat~\cite{li2023videochat} & \multicolumn{2}{c||}{-} & 50.2  & 47.0 & 65.7 & 52.5 & {51.8}\\
        & Ours & \multicolumn{2}{c||}{-} & \textbf{54.7} & \textbf{50.4} & \textbf{70.3} & \textbf{54.7} & \textbf{55.7}\\
        \hline
\end{tabular}}
}
\end{subtable}

\vspace{-4mm}
\end{table*}



==> DoraemonGPT/tables/supp_sdm_time.tex <==
\begin{table}[h]
\centering
\caption{Time Analysis of Space-Dominant Memory Construction.}
\label{tbl:supp_sdm_time}

\small
\begin{tabular}{|c|c|c|c|c|c|}
    \hline\thickhline
    \rowcolor{mygray}
Model & \makecell{ BLIP-2 \\ \cite{li2023blip}} & \makecell{ YOLO-v8 \\ \cite{yolov8}} & \makecell{ Deep OC-Sort \\ \cite{maggiolino2023deep}} & \makecell{ InternVideo \\ \cite{wang2022internvideo}} & Sum \\
    \hline\hline
Time(s) & 0.09 & 0.16 & 0.14 & 0.03 & 0.42 \\
    \hline
\end{tabular}
\end{table}

% YOLOv8~\cite{yolov8}
% Deep OC-sort~\cite{maggiolino2023deep}
% BLIP~\cite{li2022blip}/BLIP-2~\cite{li2023blip}/InstructBLIP~\cite{Dai2023InstructBLIPTG})
% InternVideo~\cite{wang2022internvideo}
% Whisper~\cite{radford2023robust}
% OCR~\cite{ocr}


==> DoraemonGPT/tables/supp_tdm_time.tex <==
\begin{table}[h]
\centering
\caption{Time Analysis of Time-Dominant Memory Construction.}
\label{tbl:supp_tdm_time}

\small
\begin{tabular}{|c|c|c|c|c|}
    \hline\thickhline
    \rowcolor{mygray}
Model & OCR~\cite{ocr} & Whisper~\cite{radford2023robust} & BLIP-2~\cite{li2023blip} & Sum  \\
    \hline\hline
Time(s) & 0.02 & 0.36 & 0.09 & 0.47 \\
    \hline
\end{tabular}
\end{table}


% YOLOv8~\cite{yolov8}
% Deep OC-sort~\cite{maggiolino2023deep}
% BLIP~\cite{li2022blip}/BLIP-2~\cite{li2023blip}/InstructBLIP~\cite{Dai2023InstructBLIPTG})
% InternVideo~\cite{wang2022internvideo}
% Whisper~\cite{radford2023robust}
% OCR~\cite{ocr}


==> DoraemonGPT/tables/supp_tvqa.tex <==
\begin{table}[h]
\centering
\small
\caption{Comparison of our DoraemonGPT with SOTAs on TVQA+~\cite{lei2020tvqa+}. $\dag$: reimplement using the officially released codes.  $*$: we filter out those failed executions (\ie, compilation error) of ViperGPT~\cite{suris2023vipergpt} and record the performance on successful executions (802/900 on \texttt{s\_val}).}
\label{tbl:supp_tvqa}

\begin{tabular}{|c|c|c|}
    \hline\thickhline
    \rowcolor{mygray}
 Method & Split & Accuracy \\
    \hline\hline
$^\dag$ViperGPT~\cite{suris2023vipergpt} & s\_val & 26.8 \\
$^{*\dag}$ViperGPT~\cite{suris2023vipergpt} & s\_val & 30.1 \\
$^\dag$VideoChat~\cite{li2023videochat} & s\_val & 34.4 \\
    \rowcolor{mygray1} DoraemonGPT & s\_val & \textbf{40.3} \\
    \hline
\end{tabular}
\end{table}


==> DoraemonGPT/tables/tvqa.tex <==
\begin{table}[h]
\vspace{-10pt}
\centering
\small
\caption{Comparison on TVQA+ \texttt{\texttt{s\_val}}.}
\label{tbl:tvqa}

\scalebox{0.88}{
\setlength\tabcolsep{4pt}
\begin{tabular}{|c|c|c|}
    \hline\thickhline
    \rowcolor{mygray}
 Method & Split & Accuracy \\
    \hline\hline
$^\dag$ViperGPT~\cite{suris2023vipergpt} & \texttt{s\_val} & 26.8 \\
$^{*\dag}$ViperGPT~\cite{suris2023vipergpt} & \texttt{s\_val} & 30.1 \\
$^\dag$VideoChat~\cite{li2023videochat} & \texttt{s\_val} & 34.4 \\
    \rowcolor{mygray1} DoraemonGPT & \texttt{s\_val} & \textbf{40.3} \\
    \hline
\end{tabular}}
\vspace{-10pt}
\end{table}

